Investigating the Impact of Model Width and Density on Generalization in Presence of Label Noise

Increasing the size of overparameterized neural networks has been a key in achieving state-of-the-art performance. This is captured by the double descent phenomenon, where the test loss follows a decreasing-increasing-decreasing pattern (or sometimes monotonically decreasing) as model width increases. However, the effect of label noise on the test loss curve has not been fully explored. In this work, we uncover an intriguing phenomenon where label noise leads to a \textit{final ascent} in the originally observed double descent curve. Specifically, under a sufficiently large noise-to-sample-size ratio, optimal generalization is achieved at intermediate widths. Through theoretical analysis, we attribute this phenomenon to the shape transition of test loss variance induced by label noise. Furthermore, we extend the final ascent phenomenon to model density and provide the first theoretical characterization showing that reducing density by randomly dropping trainable parameters improves generalization under label noise. We also thoroughly examine the roles of regularization and sample size. Surprisingly, we find that larger $\ell_2$ regularization and robust learning methods against label noise exacerbate the final ascent. We confirm the validity of our findings through extensive experiments on ReLu networks trained on MNIST, ResNets/ViTs trained on CIFAR-10/100, and InceptionResNet-v2 trained on Stanford Cars with real-world noisy labels.

==> discussion.tex <==
% \section{Discussion}

% {\bf Threshold of noise level.} Although in most of our experiments with symmetric noise the final ascent occurs only under relatively high noise levels, our finding is still practically meaningful for several reasons. Firstly, the fact that most of the recent studies on learning with label noise \citep{han2018co,zhang2018generalized,jiang2018mentornet,mirzasoleiman2020coresets,liu2020early,li2020dividemix} evaluate their methods under 60-80\% noise means that high-noise setting is indeed important to consider. Secondly, our experiments show that with asymmetric noise the required noise level is not high (Figure \ref{subfig:cifar_asym_risk}). Since asymmetric noise is often considered closer to real-world noise, the final ascent is expected to happen under moderate noise levels in realistic settings. Thirdly, applying robust methods also leads to lower required noise level (Figures \ref{subfig:elr_cifar10} and \ref{subfig:elr_cifar100}, 30-40\% noise), which is another practical scenario. \ba{we can drop if we don't have space, as this is discussed before. just add somewhere before that: asymmetric is more realistic.}


\section{Conclusion}

\yx{TODO: change conclusions based on the paper}
Our work provides new insights into the overfitting and generalization of neural networks by showing a counter example for the recently observed generalization benefits of increasing model size. We considered two ways of varying model size: changing width and randomly dropping a fraction of trainable parameters. We made two key observations: (1) when noise is sufficiently large, generalization gets worse if we increase the model size beyond some point, leading to the final ascent; (2) sufficiently large sample size can alleviate or even eliminate the final ascent. We provided theoretical evidence from random feature regression and explain such phenomenon through the lens of bias-variance decomposition. We also performed extensive experiments verifying that the above holds for neural networks. Additionally, training models with SOTA robust methods, namely ELR and DivideMix, does not mitigate the final ascent but even exacerbates it in some settings. We also provided empirical evidence which suggests the originally positive correlation between size and complexity of learned functions can be flipped by label noise. %\looseness=-1
%
While our analysis in this paper is limited to label noise, it would be valuable to investigate whether same conclusion holds for input feature noise. \looseness=-1
% \ba{use past tense in conclusion (I changed)}

